Cell Tracking according to Biological Needs -- Strong Mitosis-aware Multi-Hypothesis Tracker with Aleatoric Uncertainty

Cell tracking and segmentation assist biologists in extracting insights from large-scale microscopy time-lapse data. Driven by local accuracy metrics, current tracking approaches often suffer from a lack of long-term consistency and the ability to reconstruct lineage trees correctly. To address this issue, we introduce an uncertainty estimation technique for motion estimation frameworks and extend the multi-hypothesis tracking framework. Our uncertainty estimation lifts motion representations into probabilistic spatial densities using problem-specific test-time augmentations. Moreover, we introduce a novel mitosis-aware assignment problem formulation that allows multi-hypothesis trackers to model cell splits and to resolve false associations and mitosis detections based on long-term conflicts. In our framework, explicit biological knowledge is modeled in assignment costs. We evaluate our approach on nine competitive datasets and demonstrate that we outperform the current state-of-the-art on biologically inspired metrics substantially, achieving improvements by a factor of approximately 6 and uncover new insights into the behavior of motion estimation uncertainty.

==> tables/benchmark_technical.tex <==

\begin{table*}[t]
    \centering
    \caption{Benchmark on Technical Measures according to the \textit{CTC}~\cite{thecelltrackingchallenge}. Colored cells show the performance of top \#k state-of-the-art methods. Baseline rows compare the vanilla EmbedTrack~\cite{loeffler2022embedtrack} to the results evaluated with our approach. \textbf{Bold} numbers indicate that we outperform the baseline and \underline{underlined} numbers indicate that our approach is the new state-of-the-art. Affiliations and references for the method names can be found in Tab.~\ref{tab:tag_mapping}.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cc|ccccccccc}
            \toprule
            % ... (table headers)
            \multicolumn{2}{c}{\big[ \% \big] } & \makecell{BF-C2DL-\\HSC} & \makecell{BF-C2DL-\\MuSC} & \makecell{DIC-C2DL-\\HeLa} & \makecell{Fluo-C2DL-\\MSC} & \makecell{Fluo-N2DH-\\GOWT1} & \makecell{Fluo-N2DL-\\HeLa} & \makecell{PhC-C2DH-\\U373} & \makecell{PhC-C2DL-\\PSC} & \makecell{Fluo-N2DH-\\SIM+} \\
            \midrule
            \multirow{5}{*}{\rotatebox{90}{$\text{OP}_\text{CTB}$}} 
            & Top \#1 & 90.7
             & \cellcolor{KITGE4}87.8 & \cellcolor{MUCZ2}90.9
             & \cellcolor{BGUIL1}75.9 & \cellcolor{KTHSE1}93.8
             & \cellcolor{BGUIL5}95.6 & \cellcolor{BGUIL5}95.4 
             & \cellcolor{KITGE3}85.5 & \cellcolor{KITGE4}90.5
             \\
            & Top \#2 & \cellcolor{KITGE4}90.6 
             & 87.5 & \cellcolor{UVANL}90.4
             & \cellcolor{KTHSE1}74.0 & 94.1
             & \cellcolor{MUUS3}95.3 & \cellcolor{KITGE4}95.1
             & \cellcolor{KITGE4}85.4 & 90.3
             \\
            & Top \#3 & \cellcolor{KITGE3}90.1 
             & \cellcolor{KITGE3}87.0 & \cellcolor{MUUS2}89.8
             & \cellcolor{PURDUSAsterisk}71.0 & \cellcolor{KITGE4}94.0
             & \cellcolor{HITCN1}95.3 & \cellcolor{FRGE2}95.1
             & 85.1 & \cellcolor{UVANL}89.6
             \\
            \cmidrule(lr){2-11} 
            & Baseline & 90.6 & 87.8 & 87.9 & 63.6 & 94.0.& 94.9 & 95.1 & 85.4 & 90.5 \\
            & Ours     & \underline{\textbf{90.7}} & 87.5 & \textbf{88.3} & 62.9 & \textbf{94.1} & 94.7 & 95.1 & 85.1 & 90.3 \\
            \midrule
            \multirow{5}{*}{\rotatebox{90}{SEG}} 
            & Top \#1 & \cellcolor{KITGE4}82.6 
             & \cellcolor{KITGE4}78.2 & \cellcolor{MUCZ2}86.3
             & \cellcolor{PURDUSAsterisk}65.5 & \cellcolor{MUUS3}93.1
             & \cellcolor{MUUS3}92.3 & \cellcolor{FRGE3}92.4
             & \cellcolor{KITGE3}74.3 & \cellcolor{KITGE4}83.0
             \\
            & Top \#2 & 82.6 
             & 77.8 & \cellcolor{MUUS2}85.3
             & \cellcolor{DESUUS}64.9 & \cellcolor{KITGE4}92.9
             & \cellcolor{BGUIL5}92.2 & \cellcolor{MUUS3}92.3
             & \cellcolor{KITGE4}74.0 & 82.9
             \\
            & Top \#3 & \cellcolor{KITGE4}81.8 
             & \cellcolor{KITGE3}77.4 &  \cellcolor{UVANL}85.2
             & \cellcolor{BGUIL1}64.5 & 92.9
             & \cellcolor{HITCN1}91.9 & \cellcolor{PURDUSAsterisk}92.2
             & 73.8 & \cellcolor{MUCZ2}82.5
             \\
            \cmidrule(lr){2-11} 
            & Baseline & 82.6 & 78.2 & 82.4 & 57.9 & 92.9 & 90.6 & 92.0 & 74.0 & 83.0 \\
            & Ours     & 82.6 & 77.8 & \textbf{82.6} & 56.8 & 92.9 & 90.3 & \textbf{92.0} & 73.8 & 82.9 \\
            \midrule
            \multirow{5}{*}{\rotatebox{90}{TRA}} 
            & Top \#1 & 98.8
             & \cellcolor{KITGE4}97.4 & \cellcolor{UVANL}95.5
             & \cellcolor{BGUIL1}87.3& \cellcolor{TUGAT}97.9
             & \cellcolor{KITGE3}99.3 & \cellcolor{BGUIL5}98.5
             & \cellcolor{KITGE4}96.8 & \cellcolor{KITGE4}97.9
             \\
            & Top \#2 &  \cellcolor{PURDUSAsterisk}98.7
             & 97.1 & \cellcolor{MUCZ2}95.4
             & \cellcolor{KTHSE1}83.9 & \cellcolor{KTHSE1}97.6
             & \cellcolor{KITGE4}99.2 & \cellcolor{KITGE4}98.2
             & \cellcolor{KITGE3}96.7 & \cellcolor{BGUIL5}97.8 
             \\
            & Top \#3 & \cellcolor{KITGE3}98.5 
             & \cellcolor{KTHSE3}97.1 & \cellcolor{TUGAT}95.4
             & \cellcolor{TUGAT}78.8 & \cellcolor{BGUIL4}96.7
             & \cellcolor{RWTHGE1}99.1 & \cellcolor{NDUS1}98.2
             & \cellcolor{UVANL}96.6 & 97.7
             \\
            \cmidrule(lr){2-11} 
            & Baseline & 98.5 & 97.4 & 93.4 & 69.3 & 95.1 & 99.2 & 98.2 & 96.8 & 97.9\\
            & Ours     & \underline{\textbf{98.8}} & 97.1 & \textbf{93.9} & 69.1 & \textbf{95.3} & 99.0 & 98.1 & 96.5 & 97.7\\
            \bottomrule
        \end{tabular}

        \begin{tabular}{c}
            Method \\
            \midrule
            \cellcolor{KITGE3} KIT-GE (3) \\
            \cellcolor{KITGE4} KIT-GE (4) \\
            \cellcolor{KTHSE1} KTH-SE (1) \\
            \cellcolor{KTHSE3} KTH-SE (3) \\
            \cellcolor{BGUIL1} BGU-IL (1) \\
            \cellcolor{BGUIL4} BGU-IL (4) \\
            \cellcolor{BGUIL5} BGU-IL (5) \\
            \cellcolor{FRGE2} FR-GE (2) \\
            \cellcolor{FRGE3} FR-GE (3) \\
            \cellcolor{TUGAT} TUG-AT \\
            \cellcolor{NDUS1} ND-US (1) \\
            \cellcolor{DREXUS} DREX-US \\
            \cellcolor{UVANL} UVA-NL \\
            \cellcolor{HITCN1} HIT-CN (1) \\
            \cellcolor{RWTHGE1} RWTH-GE (1) \\
            \cellcolor{MUCZ2} MU-CZ (2) \\
            \cellcolor{PURDUSAsterisk} PURD-US (*) \\
            \cellcolor{DESUUS} DESU-US \\
            \cellcolor{MUUS2} MU-US (2) \\
            \cellcolor{MUUS3} MU-US (3) \\
            \bottomrule
        \end{tabular}
    }    
    \label{tab:benchmark_technical}
\end{table*}


==> tables/data/bio.tex <==
Dataset: BF-C2DL-HSC,BF-C2DL-MuSC,DIC-C2DL-HeLa,Fluo-C2DL-MSC,Fluo-N2DH-GOWT1,Fluo-N2DL-HeLa,PhC-C2DH-U373,PhC-C2DL-PSC,Fluo-N2DH-SIM+

Ours

CT: 0.162,0.020,0.259,0.111,0.297,0.680,0.667,0.172,0.623
TF: 0.757,0.735,0.822,0.633,0.901,0.973,0.971,0.837,0.946
BC(i): 0.564,0.680,-.---,-.---,-.---,0.869,-.---,0.596,0.914 
CCA: 0.564,0.595,-.---,-.---,-.---,0.856,-.---,0.670,0.946


KIT-GE (4)
Baseline:

CT: 0,0594	0,0100	0,1220	0,0679	0,2726	0,5876	0,5022	0,1423	0,5988
TF: 0,6226	0,6816	0,7530	0,5959	0,8400	0,9695	0,9707	0,8265	0,9366
BC(i): 0,3246	0,2468	NA	NA	NA	0,7709	NA	0,4817	0,9216
CCA: 0,1223	0,1182	NA	NA	NA	0,6275	NA	0,3475	0,8529







Competitors:
CVUT-CZ
BGU-IL (1)
DREX-US
FR-GE (2)
HD-GE (IWR)
KIT-GE (3)
KIT-GE (4)
KTH-SE (1)
KTH-SE (3)
THU-CN (2)
TUG-AT
USYD-AU
ND-US (1)
BGU-IL (1)
TUG-AT
UVA-NL
FR-GE (2)
BGU-IL (5)
HIT-CN (1)
HKI-GE
IMCB-SG (1)
KIT-GE (3)
KIT-GE (4)
KTH-SE (1)
KTH-SE (3)
KTH-SE (5)
DREX-US
KTH-SE (1*)
KTH-SE (3)
KTH-SE (5)
UVA-NL
CVUT-CZ
HD-GE (IWR)
HIT-CN (1)
KIT-GE (3)
KIT-GE (4)
UVA-NL
KTH-SE (1*)
KTH-SE (3)
KTH-SE (5)
CVUT-CZ
HD-GE (BMCV) (1)
DREX-US
HIT-CN (1)
KIT-GE (2)
KIT-GE (3)
KIT-GE (4)



==> tables/sampling_ablation.tex <==





\begin{table*}[ht]
\centering

\caption{Comparison of metrics across datasets for EmbedTrack and Ours.}
\resizebox{\linewidth}{!}{

\begin{tabular}{cc |c|c|c|c|c|c|c|c|c }
\toprule
\multicolumn{2}{c}{} &  BF-C2DL-HSC &  BF-C2DL-MuSC &  DIC-C2DH-HeLa &  Fluo-C2DL-MSC &  Fluo-N2DH-GOWT1 &  Fluo-N2DL-HeLa &  PhC-C2DH-U373 &  PhC-C2DL-PSC &  Fluo-N2DH-SIM+\\
\multirow{6 }{*}{\rotatebox{90}{  CHOTA  }}
 &  \textit{EmbedTrack} &  54.11 &  65.68 &  85.04 &  67.34 &  94.85 &  86.13 &  85.91 &  74.57 &  96.32\\
 &  \textit{EmbedTrack} x 0.5 &  39.90 &  39.11 &  84.09 &  71.04 &  94.96 &  85.57 &  85.96 &  74.94 &  96.02\\
 &  \textit{EmbedTrack} x 0.25 &  30.79 &  28.90 &  85.02 &  67.57 &  95.65 &  84.09 &  86.28 &  72.53 &  96.00\\
 &  \textit{Ours} &  76.33 &  78.45 &  87.92 &  82.98 &  95.33 &  88.67 &  86.30 &  76.72 &  96.37\\
 &  \textit{Ours} x 0.5 &  47.53 &  71.06 &  87.54 &  79.32 &  95.78 &  88.10 &  86.70 &  75.97 &  95.76\\
 &  \textit{Ours} x 0.25 &  41.30 &  52.49 &  86.06 &  75.51 &  95.61 &  84.83 &  86.90 &  72.56 &  95.41\\
\midrule
\multirow{6 }{*}{\rotatebox{90}{  TF  }}
 &  \textit{EmbedTrack} &  74.69 &  64.46 &  86.63 &  73.95 &  96.29 &  92.95 &  91.83 &  86.41 &  92.45\\
 &  \textit{EmbedTrack} x 0.5 &  44.15 &  60.95 &  87.11 &  77.00 &  97.58 &  93.38 &  91.87 &  87.99 &  94.49\\
 &  \textit{EmbedTrack} x 0.25 &  28.42 &  49.03 &  92.99 &  78.00 &  99.06 &  92.46 &  92.11 &  88.37 &  94.06\\
 &  \textit{Ours} &  93.10 &  74.57 &  89.98 &  87.49 &  96.72 &  93.93 &  88.67 &  87.67 &  93.58\\
 &  \textit{Ours} x 0.5 &  71.62 &  72.74 &  90.13 &  84.61 &  98.27 &  95.22 &  92.20 &  89.58 &  95.13\\
 &  \textit{Ours} x 0.25 &  46.74 &  67.14 &  96.24 &  77.80 &  99.15 &  93.96 &  92.11 &  89.48 &  96.32\\
\midrule
\multirow{6 }{*}{\rotatebox{90}{  CT  }}
 &  \textit{EmbedTrack} &  4.88 &  2.85 &  36.98 &  2.63 &  54.52 &  44.02 &  24.35 &  18.93 &  59.25\\
 &  \textit{EmbedTrack} x 0.5 &  1.30 &  1.60 &  38.69 &  9.52 &  62.46 &  47.97 &  30.06 &  28.47 &  68.17\\
 &  \textit{EmbedTrack} x 0.25 &  0.37 &  1.83 &  49.38 &  13.33 &  77.19 &  49.08 &  37.41 &  33.66 &  71.59\\
 &  \textit{Ours} &  29.97 &  11.95 &  55.00 &  19.35 &  51.58 &  57.42 &  30.42 &  23.27 &  58.45\\
 &  \textit{Ours} x 0.5 &  15.42 &  14.20 &  50.34 &  25.42 &  60.86 &  61.94 &  43.99 &  33.87 &  70.10\\
 &  \textit{Ours} x 0.25 &  6.26 &  8.19 &  48.53 &  26.98 &  70.25 &  58.38 &  44.82 &  36.37 &  73.16\\
\midrule
\multirow{6 }{*}{\rotatebox{90}{  CCA  }}
 &  \textit{EmbedTrack} &  12.91 &  5.65 &  N/A &  N/A &  N/A &  59.03 &  N/A &  48.42 &  87.23\\
 &  \textit{EmbedTrack} x 0.5 &  1.71 &  5.66 &  N/A &  N/A &  N/A &  62.73 &  N/A &  54.65 &  94.29\\
 &  \textit{EmbedTrack} x 0.25 &  1.24 &  6.30 &  N/A &  N/A &  N/A &  65.01 &  N/A &  57.65 &  95.31\\
 &  \textit{Ours} &  77.32 &  34.34 &  N/A &  N/A &  N/A &  86.08 &  N/A &  68.53 &  43.28\\
 &  \textit{Ours} x 0.5 &  67.60 &  40.45 &  N/A &  N/A &  N/A &  92.34 &  N/A &  77.01 &  47.06\\
 &  \textit{Ours} x 0.25 &  60.81 &  35.17 &  N/A &  N/A &  N/A &  88.55 &  N/A &  76.79 &  48.38\\
\midrule
\multirow{6 }{*}{\rotatebox{90}{  BC(0)  }}
 &  \textit{EmbedTrack} &  27.03 &  13.60 &  48.35 &  N/A &  0.00 &  60.88 &  N/A &  33.25 &  77.43\\
 &  \textit{EmbedTrack} x 0.5 &  16.30 &  17.57 &  43.45 &  N/A &  0.00 &  62.15 &  N/A &  44.72 &  84.26\\
 &  \textit{EmbedTrack} x 0.25 &  11.45 &  26.17 &  68.18 &  N/A &  0.00 &  64.53 &  N/A &  47.22 &  83.86\\
 &  \textit{Ours} &  59.90 &  43.23 &  85.42 &  N/A &  0.00 &  74.84 &  N/A &  39.97 &  78.11\\
 &  \textit{Ours} x 0.5 &  59.23 &  50.59 &  72.86 &  N/A &  0.00 &  76.31 &  N/A &  51.97 &  84.18\\
 &  \textit{Ours} x 0.25 &  46.64 &  49.39 &  67.03 &  N/A &  0.00 &  71.95 &  N/A &  51.22 &  85.26\\
\midrule
\bottomrule
\end{tabular}

}
\label{tab:comparison}
\end{table*}


==> tables/tag_mapping.tex <==
\begin{table}[t]
    \centering
    \caption{Details to related methods that are used in the main paper according to the naming conventions of the CTC~\cite{thecelltrackingchallenge}. Methods that are referenced with \textit{CTC Report} have no associated scientific publication but are described in detail in technical reports accessible at \href{http://celltrackingchallenge.net/participants/}{http://celltrackingchallenge.net/participants/}.}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{cccccc}
            \toprule
            Tag & Affiliation & Country & City & Reference \\
            \midrule
            \cellcolor{KITGE1} KIT-GE (1) & Karlsruhe Institute of Technology & Germany & Karlsruhe & \cite{StegmaierAlshutReischlMikut+2012}\\
            \cellcolor{KITGE2} KIT-GE (2) & Karlsruhe Institute of Technology & Germany & Karlsruhe & \cite{loffler2021graph}\\
            \cellcolor{KITGE3} KIT-GE (3) & Karlsruhe Institute of Technology & Germany & Karlsruhe & \cite{scherr2020cell}\\
            \cellcolor{KITGE4} KIT-GE (4) & Karlsruhe Institute of Technology & Germany & Karlsruhe & \cite{loeffler2022embedtrack}\\
            \cellcolor{KTHSE1} KTH-SE (1) & KTH Royal Institute of Technology, RaySearch Laboratories & Sweden & Stockholm & \cite{6957576}\\
            \cellcolor{KTHSE1Asterisk} KTH-SE (1*)& KTH Royal Institute of Technology, RaySearch Laboratories & Sweden & Stockholm & \cite{6957576}\\
            \cellcolor{KTHSE3} KTH-SE (3) & KTH Royal Institute of Technology, RaySearch Laboratories & Sweden & Stockholm & \cite{6957576}\\
            \cellcolor{KTHSE5} KTH-SE (5) & KTH Royal Institute of Technology, RaySearch Laboratories & Sweden & Stockholm &\cite{6957576}\\
            \cellcolor{BGUIL1} BGU-IL (1) & Ben-Gurion University of the Negev & Israel & Beer-Sheva & \cite{8759447}\\
            \cellcolor{BGUIL4} BGU-IL (4) & Ben-Gurion University of the Negev & Israel & Beer-Sheva & \cite{8759447}\\
            \cellcolor{BGUIL5} BGU-IL (5) & Ben-Gurion University of the Negev & Israel & Beer-Sheva & \cite{ben2022graph}\\%\cite{BGUIL5}\\
            \cellcolor{HDGEBMCV1} HD-GE (BMCV) (1) & Biomedical Computer Vision Group, University of Heidelberg & Germany & Heidelberg & CTC Report \\
            \cellcolor{HDGEIWR} HD-GE (IWR) & Interdisciplinary Center for Scientific Computing, University of Heidelberg & Germany & Heidelberg & \cite{Schiegg_2013_ICCV}\\
            \cellcolor{FRGE2} FR-GE (2) & University of Freiburg & Germany & Freiburg & \cite{ronneberger_u-net_2015}\\
            \cellcolor{FRGE3} FR-GE (3) & University of Freiburg & Germany & Freiburg & \cite{falk2019u} \\
            \cellcolor{HKIGE} HKI-GE (5) & Hans Knöll Institute & Germany & Jena & \cite{Belyaev2021}\\
            \cellcolor{THUCN2} THU-CN (2) & Tsinghua University & China & Beijing & \cite{10.1093/bioinformatics/btaa1106}\\
            \cellcolor{TUGAT} TUG-AT & Graz University of Technology & Austria & Graz & \cite{PAYER2019106}\\
            \cellcolor{USYDAU} USYD-AU & University of Sydney & Australia & Sydney & \cite{9434057}\\
            \cellcolor{NDUS1} ND-US (1) & University of Notre Dame & USA & Notre Dame & CTC Report\\%\cite{NDUS}\\
            \cellcolor{DREXUS} DREX-US & Drexel University & USA & Philadelphia & CTC Report\\
            \cellcolor{IMCBSG1} IMCB-SG (1) & Institute of Molecular and Cell Biology & Singapore & Singapore & CTC Report\\
            \cellcolor{UVANL} UVA-NL & University of Amsterdam & The Netherlands & Amsterdam & \cite{gupta2019tracking}\\
            \cellcolor{HITCN1} HIT-CN (1) & Harbin Institute of Technology & China & Shenzhen & \cite{zhou2019joint}\\
            \cellcolor{CVUTCZ} CVUT-CZ & Czech Technical University in Prague & Czech Republic & Prague & \cite{sixta2020coupling} \\
            \cellcolor{RWTHGE1} RWTH-GE (1) & RWTH Aachen University & Germany & Aachen & \cite{8759242}\\
            \cellcolor{MUCZ2} MU-CZ (2) & Masaryk University & Czech Republic & Brno & \cite{lux2020cell}\\
            \cellcolor{PURDUSAsterisk} PURD-US (*) & Purdue University & USA & West Lafayette & \cite{guo2022training}\\
            \cellcolor{DESUUS} DESU-US & Delaware State University & USA & Dover & CTC Report\\
            \cellcolor{MUUS2} MU-US (2) & University of Missouri & USA & Columbia & CTC Report \\
            \cellcolor{MUUS3} MU-US (3) & University of Missouri & USA & Columbia & \cite{Bao_2021_ICCV} \\
            \bottomrule
        \end{tabular}
    }    
    \label{tab:tag_mapping}
\end{table}
